Transformer-Based Models Are Not Yet Perfect At Learning to Emulate Structural Recursion

This paper investigates the ability of transformer-based models to learn structural recursion from examples. Recursion is a universal concept in both natural and formal languages. Structural recursion is central to the programming language and formal mathematics tasks where symbolic tools currently excel beyond neural models, such as inferring semantic relations between datatypes and emulating program behavior. We introduce a general framework that nicely connects the abstract concepts of structural recursion in the programming language domain to concrete sequence modeling problems and learned models' behavior. The framework includes a representation that captures the general \textit{syntax} of structural recursion, coupled with two different frameworks for understanding their \textit{semantics} -- one that is more natural from a programming languages perspective and one that helps bridge that perspective with a mechanistic understanding of the underlying transformer architecture. With our framework as a powerful conceptual tool, we identify different issues under various set-ups. The models trained to emulate recursive computations cannot fully capture the recursion yet instead fit short-cut algorithms and thus cannot solve certain edge cases that are under-represented in the training distribution. In addition, it is difficult for state-of-the-art large language models (LLMs) to mine recursive rules from in-context demonstrations. Meanwhile, these LLMs fail in interesting ways when emulating reduction (step-wise computation) of the recursive function.

==> conclusions.tex <==
\section{Conclusions, Limitations, and Future Work}
\label{sec:conclusions}

Transformer models can approximate the behavior of
important structurally recursive functions,
but the shortcuts they learn fall short.
We have shown that, by reconstructing the
algorithms corresponding to these shortcuts,
it is possible to understand and even predict
\textit{how} and \textit{why} they fall short. In this work, our main focus was on toy transformer models trained from scratch, while we deferred the understanding of large pretrained language models to future work.
One next step is to use similar analyses
to understand the shortcomings of large pretrained language models on programming and reasoning tasks, and to make sense of why tricks like chain of thought reasoning and scratchpadding help on those tasks. Beyond that, we are excited to use our
newfound understanding to drive future improvements to training and prompting techniques, neural architectures, and evaluation methodologies.

% \section*{Acknowledgement}
% We would like to thank Chris Olah, Jason Rute, Nadia Polikarpova and Neel Nanda for their valuable inputs.

==> construction.tex <==
% \section{Discussion: Construction of Transformers that perform reductions }

% Transformers are shown to be constructed to achieve Turing completeness. \Dylan{Cite}

% In fact, one can construct a single-layer casual transformer that performs one-step reduction for binary successor tasks. By stacking these layers and implementing a simple mechanism that checks the convergence of the algorithm (i.e. searching for the existence of \texttt{S} symbol), such a model can compute the successor of a binary string requiring recursive depth $D$ in the constructor notation with $D$ layers.

% In addition, it it amenable to construct transformer models to perform the entire computation for the binary successor problem up to a bounded length by searching for consecutive \texttt{X1}'s at the end and deciding whether to produce an \texttt{X1} then copy the rest, or \texttt{X0 01} based on the succeeding entry of the deepest \texttt{X1}.


% In addition, building upon existing works on Dyck language generation, it can also be straightforward to prove the existence of models that perform one-step reduction on the task of tree traversal by adding layers that copy node values with pre-labeled depts of parentheses.



==> metadata.tex <==

$plots/attn_bin_nat/depth0_layer_0_head_0? enc-dec, 128, 2 heads, lr=1 $
